Instance-Aware Image Completion

Image completion is a task that aims to fill in the missing region of a masked image with plausible contents. However, existing image completion methods tend to fill in the missing region with the surrounding texture instead of hallucinating a visual instance that is suitable in accordance with the context of the scene. In this work, we propose a novel image completion model, dubbed ImComplete, that hallucinates the missing instance that harmonizes well with - and thus preserves - the original context. ImComplete first adopts a transformer architecture that considers the visible instances and the location of the missing region. Then, ImComplete completes the semantic segmentation masks within the missing region, providing pixel-level semantic and structural guidance. Finally, the image synthesis blocks generate photo-realistic content. We perform a comprehensive evaluation of the results in terms of visual quality (LPIPS and FID) and contextual preservation scores (CLIPscore and object detection accuracy) with COCO-panoptic and Visual Genome datasets. Experimental results show the superiority of ImComplete on various natural images.

==> sections/architectures.tex <==
\clearpage
\chapter{Network Architectures}
\sloppy

We implement our completion model for experiments using PyTorch~\cite{NEURIPS2019_9015} library. We use PyTorch functions and define some necessary notations here to provide the architectural details of \OursAcronym{}.

\textsc{Embedding}($dim_{out}$) indicates PyTorch embedding function. \textsc{TransEncLayer}($dim_{token}, dim_{hidden}, head_{numb}$) is a vanilla transformer encoder layer. \textsc{FC($dim_{input}, dim_{output}$)} is a single linear layer. \textsc{Conv}($kernel_{size}, stride, padding$) is a convolution layer. \textsc{DBlock}($channel_{in}, channel_{out}, downsampling$) and \textsc{BigGBlock}($channel_{in}, channel_{out}, upsampling, dim_{z_{split}}, dim_{shared}$) are BigGAN blocks implemented in StudioGAN libary~\cite{kang2022studiogan}. \textsc{Self-Attention} is a self-attention block implemented in StudioGAN. \textsc{BN} and \textsc{LN} indicate a batch normalization and layer normalization layer, respectively. \textsc{SPADEResnetBlock} is a SPADE block~\cite{park2019SPADE}. \textsc{ResBlock-Up} and -\textsc{Down} indicate ResNet blocks implemented in StudioGAN. \textsc{Up($size$)} indicates a upsampling function PyTorch provides. N is the number of classes in the segmentation mask. m and k indicate the batch size and the number of visible instances for a given masked image.

\input{assets/tables/MITArchitecture.tex}
\input{assets/tables/ISGArchitecture.tex}
\input{assets/tables/BSCArchitecture.tex}
\input{assets/tables/SISGArchitecture.tex}
\input{assets/tables/SISDArchitecture.tex}

